An Empirical Comparison of Pre-Trained Models of Source Code

While a large number of pre-trained models of source code have been successfully developed and applied to a variety of software engineering (SE) tasks in recent years, our understanding of these pre-trained models is arguably fairly limited. With the goal of advancing our understanding of these models, we perform the first systematic empirical comparison of 19 recently-developed pre-trained models of source code on 13 SE tasks. To gain additional insights into these models, we adopt a recently-developed 4-dimensional categorization of pre-trained models, and subsequently investigate whether there are correlations between different categories of pre-trained models and their performances on different SE tasks.

==> tables/architecture_compare.tex <==
\begin{table}[t!]
    \centering
    %\scriptsize
    \caption{Results of TE-, TD- and TF-based models on SE tasks.}
    \label{table:architecture_compare}
    \resizebox{0.68\linewidth}{!}{%
    \begin{NiceTabular}{lrrr|rrr}
    \CodeBefore
        \rowcolors{3}{}{gray!15}[respect-blocks]
    \Body
        \toprule
            \Block{2-1}{} &
            \Block{1-3}{\textbf{Current results}} &
            &
            &
            \Block{1-3}{\textbf{New results}} &
            &
            \\
        \cline{2-7}
            & 
            \Block[c]{}{\textbf{TE}} &
            \Block[c]{}{\textbf{TD}} &
            \Block[c]{}{\textbf{TF}} &
            \Block[c]{}{\textbf{TE}} &
            \Block[c]{}{\textbf{TD}} &
            \Block[c]{}{\textbf{TF}} \\
        \midrule
            DD   & 
                60.95          & -              & \textbf{64.98} & 
                \textbf{64.98} & 64.71          & 64.62          \\
            CD   & 
                96.57          & -              & \textbf{96.77} & 
                96.32          & 96.06          & \textbf{96.47} \\
            ET   & 
                79.12 & -              & -              & 
                \textbf{78.98}         & 77.49          & 77.45          \\
            CR   & 
                86.65          & -              & -              & 
                82.87          & 63.93          & \textbf{83.64} \\
            CS   & 
                \textbf{41.30} & -              & 38.2           & 
                33.42          & 25.18          & \textbf{37.59} \\
            QA   & 
                \textbf{68.07} & -              & 66.4           & 
                62.32          & 52.28          & \textbf{63.75} \\
            CT   & 
                59.48          & -              & \textbf{64.46} & 
                60.42          & 60.70          & \textbf{64.67} \\
            BF   & 
                12.00          & -              & \textbf{14.16} & 
                13.17          & 11.50          & \textbf{15.38} \\
            CC   & 
                -              & 42.37          & -              & 
                40.72          & \textbf{43.31} & 40.14          \\
            MG   & 
                -              & -              & 28.00 & 
                28.36          & 27.44          & \textbf{31.64} \\
            AG   & 
                -              & -              & 40.50 & 
                45.67          & 45.27          & \textbf{48.52} \\
            CS   & 
                18.57          & -              & \textbf{18.69} & 
                17.51          & 16.79          & \textbf{18.34} \\
            CG   & 
                \textbf{22.60} & 20.10          & 20.38          & 
                20.66          & 20.00          & \textbf{20.72} \\
        \hline
            Avg. & -     & -     & -     & 49.64 & 46.51 & \textbf{51.00} \\
        \bottomrule
    \end{NiceTabular}
     }%
\end{table}

==> tables/codeptms_short.tex <==
\begin{table}[t]
	\centering
	\caption{Categorization of existing pre-trained models.}
	\label{table:codeptms}
	\resizebox{\linewidth}{!}{%
	\begin{NiceTabular}{lllll}
	\CodeBefore
	    \rowcolors{2}{gray!15}{}
	\Body
	    \toprule
            \textbf{Models} &
            \textbf{Arch.} &
            \textbf{Modality} &
            \textbf{Objective} &
            \textbf{PL} \\
        \midrule
            RoBERTa~\cite{liu2019roberta} &
            TE &
            NL Text &
            MLM &
            - \\
        GPT-2~\cite{radford2019gpt2} &
            TD &
            NL Text &
            ULM &
            - \\
        BART~\cite{lewis2020bart} &
            TF &
            NL Text &
            DAE &
            - \\
        T5~\cite{raffel2020t5} &
            TF &
            NL Text &
            Seq2Seq MLM &
            - \\
        \hline
            SCELMo~\cite{karampatsis2020scelmo} &
            LSTM &
            Code &
            BiLM &
            Mono \\
        CuBERT~\cite{kanade2020cubert} &
            TE &
            Code &
            MLM + NSP &
            Mono \\
        GPT-C~\cite{svyatkovskiy2020gpt-c} &
            TD &
            Code &
            ULM &
            Multi \\
        C-BERT~\cite{buratti2020c-bert} &
            TE &
            Code &
            MLM &
            Mono \\
        JavaBERT~\cite{de2021javabert} &
            TE &
            Code &
            MLM &
            Mono \\
        CodeGPT-adapted~\cite{lu2021codexglue} &
            TD &
            Code &
            ULM & 
            Multi \\
        DeepDebug~\cite{drain2021deepdebug} &
            TF &
            Code &
            Seq2Seq MLM &
            Mono \\
        \hline
            CodeBERT~\cite{feng2020codebert} &
            TE &
            Code + Doc &
            MLM \& RTD &
            Multi \\
        GraphCodeBERT~\cite{guo2021graphcodebert} &
            TE &
            \Block{}{Code + Doc +\\ DFG Nodes} &
            \Block{}{MLM + EP + NA} &
            Multi \\
        CugLM~\cite{liu2020cuglm} &
            TE &
            Code &
            \Block{}{IMLM + NSP + ULM} &
            Multi \\
        DOBF~\cite{roziere2021dobf} &
            TF &
            Code &
            \Block{}{MLM \& Seq2Seq IMLM} &
            Multi \\
        T5-learning~\cite{mastropaolo2021t5-learning} &
            TF &
            Code \& Doc &
            Seq2Seq MLM &
            Mono \\
        PLBART~\cite{ahmad2021plbart} &
            TF &
            Code \& Post &
            DAE &
            Multi \\
        ProphetNet-Code~\cite{qi2021prophetnet-code} &
            TF &
            Code \& Doc &
            FNP &
            Multi \\
        CoTexT~\cite{phan2021cotext} &
            TF &
            Code + Doc &
            Seq2Seq MLM &
            Multi \\
        TreeBERT~\cite{jiang2021treebert} &
            TF &
            \Block{}{Code +\\ AST Paths} &
            TMLM + NOP &
            Multi \\
        OSCAR~\cite{peng2021oscar} &
            TE &
            IR + AEI &
            MLM + CCL &
            Mono \\
        CodeDisen~\cite{zhang2021codedisen} &
            LSTM &
            \Block{}{Code +\\ AST Seq} &
            \Block{}{VGVAE + CLR\\ + PD + ACP} &
            Multi \\
        CodeT5~\cite{wang2021codet5} &
            TF &
            Code + Doc &
            \Block{}{Seq2Seq MLM / IT /\\ Seq2Seq IMLM / BDG} &
            Multi \\
        SynCoBERT~\cite{wang2021syncobert} &
            TE &
            \Block{}{Code + Doc +\\ AST Seq} &
            \Block{}{MLM + IT + TEP +\\ MCL} &
            Multi \\
        SPT-Code~\cite{niu2022sptcode} &
            TF & 
            \Block{}{Code +\\ Names +\\ AST Seq} &
            \Block{}{CAP \& MASS \& MNG} &
            Multi \\
        UniXcoder~\cite{guo2022unixcoder} &
            TE & 
            \Block{}{AST Seq +\\ Doc} &
            \Block{}{MLM / ULM / Seq2Seq\\ MLM / MCL / CMG} &
            Multi \\
        \bottomrule
    \end{NiceTabular}%
    }
\end{table}

==> tables/modality_compare.tex <==
\begin{table}[t!]
    \centering
    % \scriptsize
    \caption{Results of five categories on modalities on SE tasks.}
    \label{table:modality_compare}
    \resizebox{\linewidth}{!}{%
    \begin{NiceTabular}{lrrr|rr|rrr|rr}
    \CodeBefore
        \rowcolors{3}{}{gray!15}[respect-blocks]
    \Body
        \toprule
            \Block{2-1}{} &
            \Block{1-5}{\textbf{Current results}} &
            &
            &
            &
            &
            \Block{1-5}{\textbf{New results}} &
            &
            &
            &
            \\
        \cline{2-11}
            & 
            \Block[c]{}{\textbf{C}} &
            \Block[c]{}{\textbf{NL}} &
            \Block[c]{}{\textbf{S}} &
            \Block[c]{}{\textbf{+}} &
            \Block[c]{}{\textbf{\&}} &
            \Block[c]{}{\textbf{C}} &
            \Block[c]{}{\textbf{NL}} &
            \Block[c]{}{\textbf{S}} &
            \Block[c]{}{\textbf{+}} &
            \Block[c]{}{\textbf{\&}} \\
        \midrule
            DD   & 
                57.40 & \textbf{64.86} & 64.50 & 
                \textbf{65.42} & 63.18 & 
                64.31 & 65.06 & \textbf{65.69} & 
                \textbf{65.62} & 63.79 \\
            CD   & 
                95.90 & \textbf{96.82} & 96.57 & 
                96.73 & \textbf{97.20} & 
                95.96 & 96.67 & \textbf{96.78} & 
                \textbf{96.73} & 96.48 \\
            ET   & 
                79.12 & -     & -     & 
                -     & -     & 
                76.08 & 79.72 & \textbf{80.92} & 
                \textbf{81.01} & 75.72 \\
            CR   & 
                -     & 86.65 & \textbf{87.97} & 
                86.65 & -     & 
                74.90 & 85.88 & \textbf{87.78} & 
                \textbf{87.33} & 81.89 \\
            CS   & 
                38.30 & 39.70 & \textbf{41.30} & 
                39.70 & -     & 
                28.54 & 38.81 & \textbf{39.39} & 
                \textbf{39.17} & 38.11 \\
            QA   & 
                -     & 67.40 & \textbf{69.25} & 
                \textbf{68.00} & 65.00 & 
                55.99 & 66.41 & \textbf{67.51} & 
                \textbf{67.51} & 62.98 \\
            CT   & 
                -     & \textbf{61.97} & 60.71 & 
                61.41 & \textbf{64.80} & 
                60.02 & \textbf{64.35} & 63.74 & 
                63.96 & \textbf{64.98} \\
            BF   & 
                15.05 & 13.41 & \textbf{13.70} & 
                \textbf{14.66} & 10.30 & 
                12.24 & 15.21 & \textbf{15.58} & 
                \textbf{15.68} & 14.50 \\
            CC   & 
                42.37 & -     & -     & 
                -     & -     & 
                40.89 & 40.48 & \textbf{41.08} & 
                \textbf{40.88} & 39.82 \\
            MG   & 
                -     & 28.00 & -     & 
                -     & 28.00 & 
                27.89 & 31.03 & \textbf{31.11} & 
                \textbf{31.36} & 30.87 \\
            AG   & 
                -     & 40.50 & -     & 
                -     & 40.50 & 
                45.66 & 47.75 & \textbf{47.98} &
                47.71 & \textbf{48.55} \\
            CS   & 
                18.65 & 18.65 & \textbf{19.30} & 
                \textbf{18.77} & 18.43 & 
                16.99 & \textbf{18.45} & 18.42 & 
                \textbf{18.56} & 18.09 \\
            CG   & 
                20.10 & 20.94 & \textbf{22.60} & 
                \textbf{21.67} & 18.75 & 
                19.73 & 21.19 & \textbf{21.41} & 
                \textbf{21.68} & 20.17 \\
        \hline
            Avg. & -     & -     & -     & 
                -     & -     & 
                47.63 & 51.60 & \textbf{52.10} & 
                \textbf{52.09} & 50.46 \\
        \bottomrule
    \end{NiceTabular}
    }%
\end{table}

==> tables/objective_compare.tex <==
\begin{table}[t!]
    \centering
    % \scriptsize
    \caption{Results of five categories on pre-training objective on SE tasks.}
    \label{table:objective_compare}
    \resizebox{\linewidth}{!}{%
    \begin{NiceTabular}{lrr|rrr|rr|rrr}
    \CodeBefore
        \rowcolors{3}{}{gray!15}[respect-blocks]
    \Body
        \toprule
            \Block{2-1}{} &
            \Block{1-5}{\textbf{Current results}} &
            &
            &
            &
            &
            \Block{1-5}{\textbf{New results}} &
            &
            &
            &
            \\
        \cline{2-11}
            & 
            \Block[c]{}{\textbf{NLP}} &
            \Block[c]{}{\textbf{SE}} &
            \Block[c]{}{\textbf{+}} &
            \Block[c]{}{\textbf{\&}} &
            \Block[c]{}{\textbf{/}} &
            \Block[c]{}{\textbf{NLP}} &
            \Block[c]{}{\textbf{SE}} &
            \Block[c]{}{\textbf{+}} &
            \Block[c]{}{\textbf{\&}} &
            \Block[c]{}{\textbf{/}} \\
        \midrule
            DD   & 
                62.19 & \textbf{65.14} & 
                \textbf{64.50} & -     & 64.48 & 
                64.41 & \textbf{65.29} & 
                \textbf{65.27} & 64.59 & 65.22 \\
            CD   & 
                \textbf{97.20} & 96.56 & 
                \textbf{97.25} & 95.90 & 96.53 & 
                96.05 & \textbf{96.79} & 
                96.48 & 96.67 & \textbf{96.84} \\
            ET   & 
                79.12 & -     & 
                79.12 & -     & -     & 
                76.02 & \textbf{80.96} & 
                80.59 & 79.13 & \textbf{82.13} \\
            CR   & 
                82.67 & \textbf{87.97} & 
                86.70 & 82.67 & \textbf{90.52} & 
                76.96 & \textbf{87.13} & 
                84.40 & 86.49 & \textbf{87.70} \\
            CS   & 
                -     & 39.23 & 
                -     & 38.30 & \textbf{39.70} & 
                31.29 & \textbf{38.97} & 
                35.36 & 37.94 & \textbf{40.10} \\
            QA   & 
                65.35 & \textbf{68.77} & 
                \textbf{68.40} & 65.70 & 67.63 & 
                58.97 & \textbf{66.03} & 
                63.70 & 63.92 & \textbf{67.74} \\
            CT   & 
                61.65 & \textbf{62.13} & 
                59.98 & 60.34 & \textbf{65.60}  & 
                61.40 & \textbf{63.92} & 
                61.19 & 63.53 & \textbf{66.22} \\
            BF   & 
                12.75 & \textbf{15.06} & 
                13.20 & 12.50 & \textbf{15.94} & 
                13.33 & \textbf{15.02} & 
                13.88 & 13.46 & \textbf{16.57} \\
            CC   & 
                42.37 & -     & 
                -     & -     & -     & 
                40.49 & \textbf{41.03} & 
                40.95 & 40.11 & \textbf{41.32} \\
            MG   & 
                28.00 & -     & 
                -     & -     & -     & 
                29.08 & \textbf{30.83} & 
                29.39 & 30.26 & \textbf{32.56} \\
            AG   & 
                40.50 & -     & 
                -     & -     & -     & 
                46.40 & \textbf{47.77} & 
                46.60 & 47.63 & \textbf{48.64} \\
            CS   & 
                18.27 & \textbf{19.17} & 
                -     & 18.24 & \textbf{19.06} & 
                17.42 & \textbf{18.38} & 
                17.66 & 18.13 & \textbf{18.96} \\
            CG   & 
                19.65 & \textbf{22.45} & 
                -     & -     & 21.22 & 
                19.92 & \textbf{21.58} & 
                21.05 & 20.50 & \textbf{21.97} \\
        \hline
            Avg. & 
                -     & -     & 
                -     & -     & -     & 
                48.60 & \textbf{51.82} & 
                50.50 & 50.95 & \textbf{52.77} \\
        \bottomrule
    \end{NiceTabular}
    }%
\end{table}

==> tables/pl_compare.tex <==
\begin{table}[t!]
    \centering
    %\scriptsize
    \caption{Results of Monolingual and Multilingual models on SE tasks.}
    \label{table:pl_compare}
    \resizebox{0.74\linewidth}{!}{%
    \begin{NiceTabular}{lrrr|rrr}
    \CodeBefore
        \rowcolors{3}{}{gray!15}[respect-blocks]
    \Body
        \toprule
            \Block{2-1}{} &
            \Block{1-3}{\textbf{Current results}} &
            &
            &
            \Block{1-3}{\textbf{New results}} &
            &
            \\
        \cline{2-7}
            &
            \Block[c]{}{\textbf{Mono.}} &
            \Block[c]{}{\textbf{Multi.}} &
            \Block[c]{}{\textbf{ER}} &
            \Block[c]{}{\textbf{Mono.}} &
            \Block[c]{}{\textbf{Multi.
                }} &
            \Block[c]{}{\textbf{ER}} \\
        \midrule
            DD   & 
                57.40 & 64.86 & -21.23 & 
                64.12 & 65.02 & -2.57  \\
            CD   & 
                -     & 96.67 & -      & 
                95.73 & 96.59 & -25.31  \\
            ET   & 
                79.12 & -     & -      & 
                73.10 & 79.89 & -33.76  \\
            CR   & 
                -     & 86.65 & -      & 
                76.31 & 83.00 & -39.35  \\
            CS   & 
                -     & 39.23 & -      & 
                28.24 & 36.77 & -13.50 \\
            QA   & 
                -     & 67.40 & -      & 
                56.16 & 64.01 & -21.82 \\
            CT   & 
                -     & 61.97 & -      & 
                59.34 & 63.58 & -11.63  \\
            BF   & 
                10.78 & 14.56 & -4.42 & 
                12.98 & 14.42 & -1.69  \\
            CC   & 
                -     & 42.37 & -      & 
                39.26 & 41.24 & -3.37  \\
            MG   & 
                28.00 & -     & -      & 
                28.37 & 30.34 & -2.44  \\
            AG   & 
                40.50 & -     & -      & 
                46.03 & 47.32 & -2.82  \\
            CS   & 
                -     & 18.65 & -      & 
                16.87 & 18.17 & -1.59  \\
            CG   & 
                -     & 20.77 & -      & 
                18.93 & 21.22 & -2.91 \\
        \hline
            Avg. & -     & -     & -      & 47.34 & 50.89 & -7.23  \\
        \bottomrule
    \end{NiceTabular}
    }%
\end{table}
